CuraWeb: Joint Optimization of Quality, Redundancy, and Diversity for Web-Scale Pretraining Data

Open-web corpora curated via highly selective filters, such as FineWeb-Edu and DCLM, constitute the core of LLM pretraining data and have significantly advanced LLM performance. However, these pipelines typically rely on singular optimization objectives, which inevitably narrows distributional diversity and marginalizes long-tail knowledge, thereby restricting data coverage and underutilizing the vast potential of the open web. To address this limitation, we propose a novel curation paradigm that shifts from linear pruning to the joint optimization of quality, redundancy, and diversity. This framework synergizes dual-track cleaning (rule-based and model-driven) with hybrid deduplication (n-gram and semantic), while employing a multi-objective sampler to balance informational quality with distributional breadth. Applying this framework to Common Crawl, we construct CuraWeb, a 2T-token English corpus. Unlike existing resources, CuraWeb establishes an industrial-grade standard for data curation by recovering a more holistic data distribution with enhanced diversity and minimal redundancy, achieving broader coverage of long-tail knowledge across diverse domains. Experimental evaluations at the 3B scale demonstrate that CuraWeb significantly outperforms state-of-the-art baselines, yielding an average performance gain of 1.8\% across a wide range of benchmarks, particularly in knowledge-intensive and reasoning tasks.

==> Tables/Dataset-Preparation.tex <==
\begin{table}[h] 
\centering      
\caption{Data funnel across the LongCat-CC pipeline. Document counts are reported after each processing stage.}  
\label{tab:funnel} 
\begin{tabular}{lrr}  
\toprule
\textbf{Stage} & \textbf{Output Documents} & \textbf{Retention} \\
\midrule 
Raw Common Crawl (2013--2024) & 184,888,259,093 & --- \\ 
Exact Deduplication            & 41,418,969,866  & 22.4\% \\
URL Filtering                  & 39,141,282,466  & 94.5\% \\ 
Rule-Based Filtering           & 34,184,934,711  & 87.3\% \\ 
Model-Based Filtering          & 23,293,962,960  & 68.1\% \\ 
Fuzzy Deduplication            & 7,970,003,383   & 34.2\% \\ 
Semantic Deduplication         & 6,424,597,993   & 80.6\% \\ 
Quality-Diversity Sampling     & 2,402,967,760   & 30.2\% \\ 
\bottomrule                                                                           
\end{tabular}                                                                         
\end{table} 

==> Tables/Rule-based-filtering.tex <==
\begin{table}[t]
  \centering
  \caption{Rule-based filter removal rates measured on a 10\% corpus sample across production months 4 through 7.}
  \label{tab:rules}
  \begin{tabularx}{\linewidth}{lrX}
  \toprule
  \textbf{Rule} & \textbf{Removal Rate} & \textbf{Description} \\
  \midrule
  Required word count $<$ 2         & 31.98\% & Removes documents with fewer than two function words, indicating non-natural language. \\
  Duplicate 5-gram ratio $>$ 0.15   & 28.74\% & Removes documents where more than 15\% of characters fall within repeated 5-grams. \\
  Alphabetic character ratio $<$ 0.8 & 28.20\% & Removes documents with insufficient alphabetic content. \\
  Boilerplate classifier score $>$ 0.9 & 27.47\% & Removes pages dominated by low-quality templated content such as headers and footers. \\
  Word count $<$ 50                 & 25.86\% & Removes documents that are too short to contain meaningful content. \\
  \bottomrule
  \end{tabularx}
\end{table}


==> Tables/Semantic-deduplication.tex <==
\begin{table}[h]
\centering
\caption{Representative high-redundancy clusters identified by semantic deduplication. Redundancy rate is the fraction of within-cluster documents removed.}                          
\label{tab:semdedup_clusters}
\begin{tabular}{lrr}
\toprule    
\textbf{Cluster Type} & \textbf{Documents} & \textbf{Redundancy Rate} \\
\midrule 
South African Tax Calculations  & 46,781  & 99.96\% \\
Switzerland Salary Calculations & 183,436 & 97.69\% \\
Japan Income Tax Calculations   & 117,579 & 98.37\% \\
Monthly Weather Forecast Pages  & 183,436 & 97.69\% \\
Hex Color Code Documentation    & 96,175  & 94.26\% \\
Currency Exchange Rate Pages    & 157,000 & 82.32\% \\
Academic Library Database Guides & 84,195 & 83.34\% \\ 
\bottomrule
\end{tabular} 
\end{table}
